Improving Language Model Personas via Rationalization with Psychological Scaffolds

Language models prompted with a user description or persona are being used to predict the user's preferences and opinions. However, existing approaches to building personas mostly rely on a user's demographic attributes and/or prior judgments, but not on any underlying reasoning behind a user's judgments. We introduce PB&J (Psychology of Behavior and Judgments), a framework that improves LM personas by incorporating potential rationales for why the user could have made a certain judgment. Our rationales are generated by a language model to explicitly reason about a user's behavior on the basis of their experiences, personality traits, or beliefs. Our method employs psychological scaffolds: structured frameworks such as the Big 5 Personality Traits or Primal World Beliefs to help ground the generated rationales in existing theories. Experiments on public opinion and movie preference prediction tasks demonstrate that language model personas augmented with PB&J rationales consistently outperform personas conditioned only on user demographics and / or judgments, including those that use a model's default chain-of-thought, which is not grounded in psychological theories. Additionally, our PB&J personas perform competitively with those using human-written rationales, suggesting the potential of synthetic rationales guided by existing theories.

==> latex/figures/prompt_big5.tex <==
\begin{figure}[!h]
\small
% \begin{framed}
% Category: \\
% Views on gender \\

\begin{mdframed}[linecolor=black!30,backgroundcolor=black!5]
\textbf{System Message:}

A person can be described as follows: \\
\\
<demographic information>\\

The person has the following judgements:

1. <judgement\_1>\\
2. <judgement\_2>\\
3. <judgement\_3>\\
\end{mdframed}

\begin{mdframed}[linecolor=black!30,backgroundcolor=red!5]
\textbf{User Message}\\

For a given judgement, what would be a brief, reasonable explanation that the person would provide for holding that judgement? The explanation should be grounded in the big five personality traits listed below:\\
            
1. Openness to experience (includes aspects such as intellectual curiosity and creative imagination)\\
2. Conscientiousness (organization, productiveness, responsibility)\\
3. Extroversion (sociability, assertiveness; its opposite is Introversion)\\
4. Agreeableness (compassion, respectfulness, trust in others)\\
5. Neuroticism (tendencies toward anxiety and depression)\\

Judgement: <judgement\_i>
\end{mdframed}

\caption{\brihi{add caption}}
\label{fig:prompt_big5}
\end{figure}


==> latex/figures/prompt_experience.tex <==
\begin{figure}[!h]
\small
% \begin{framed}
% Category: \\
% Views on gender \\

\begin{mdframed}[linecolor=black!30,backgroundcolor=black!5]
\textbf{System Message:}

A person can be described as follows: \\
\\
<demographic information>\\

The person has the following judgements:

1. <judgement\_1>\\
2. <judgement\_2>\\
3. <judgement\_3>\\
\end{mdframed}

\begin{mdframed}[linecolor=black!30,backgroundcolor=red!5]
\textbf{User Message}\\

For a given judgement, what would be a reasonable explanation that the person would provide for holding that judgement? The explanation should contain a specific experience or personality trait (for example, fill in details of the university, or food, or any other detail, that the person would use to better explain their judgment).\\

Judgement: <judgement\_i>
\end{mdframed}

\caption{\brihi{add caption}}
\label{fig:prompt_experience}
\end{figure}


==> latex/figures/prompt_noinstruct_generation.tex <==
\begin{figure}[!h]
\small
% \begin{framed}
% Category: \\
% Views on gender \\

\begin{mdframed}[linecolor=black!30,backgroundcolor=black!5]
\textbf{System Message:}

A person can be described as follows: \\
\\
<demographic information>\\

The person has the following judgements:

1. <judgement\_1>\\
2. <judgement\_2>\\
3. <judgement\_3>\\
\end{mdframed}

\begin{mdframed}[linecolor=black!30,backgroundcolor=red!5]
\textbf{User Message}\\

For a given judgement, what would be a reasonable explanation that the person would provide for holding that judgement?\\

Judgement: <judgement\_i>
\end{mdframed}

\caption{\brihi{add caption}}
\label{fig:prompt_noinstruct}
\end{figure}


==> latex/figures/prompt_primalbeliefs.tex <==
\begin{figure}[!h]
\small
% \begin{framed}
% Category: \\
% Views on gender \\

\begin{mdframed}[linecolor=black!30,backgroundcolor=black!5]
\textbf{System Message:}

A person can be described as follows: \\
\\
<demographic information>\\

The person has the following judgements:

1. <judgement\_1>\\
2. <judgement\_2>\\
3. <judgement\_3>\\
\end{mdframed}

\begin{mdframed}[linecolor=black!30,backgroundcolor=red!5]
\textbf{User Message}\\

For a given judgement, what would be a brief, reasonable explanation that the person would provide for holding that judgement? The explanation should be grounded in the three primal world beliefs listed below:\\
            
1. Safe World Belief: Those low on Safe see a Hobbesian world defined by misery, decay, scarcity, brutality, and dangers of all sorts. Those high on Safe see a world of cooperation, comfort, stability, and few threats.\\
2. Enticing World Belief: Those low on Enticing inhabit dull and ugly worlds where exploration offers low return on investment. Those high on Enticing inhabit an irresistibly fascinating reality.\\
3. Alive World Belief: Those low on Alive inhabit inanimate, mechanical worlds without awareness or intent. Those high on Alive sense that everything happens for a purpose and are thus sensitive to those purposes.\\

Judgement: <judgement\_i>
\end{mdframed}

\caption{\brihi{add caption}}
\label{fig:prompt_primalbelief}
\end{figure}


==> latex/figures/prompt_shwartz.tex <==
\begin{figure}[!h]
\small
% \begin{framed}
% Category: \\
% Views on gender \\

\begin{mdframed}[linecolor=black!30,backgroundcolor=black!5]
\textbf{System Message:}

A person can be described as follows: \\
\\
<demographic information>\\

The person has the following judgements:

1. <judgement\_1>\\
2. <judgement\_2>\\
3. <judgement\_3>\\
\end{mdframed}

\begin{mdframed}[linecolor=black!30,backgroundcolor=red!5]
\textbf{User Message}\\

For a given judgement, what would be a brief, reasonable explanation that the person would provide for holding that judgement? The explanation should be grounded in the Shwartz Theory of Basic Human Values listed below: \\
            
1. Power: Refers to the pursuit of social status, dominance, and control over people and resources.\\
2. Achievement: Personal pursuit of success, demonstrating competence according to social standards.\\
3. Hedonism: Pursuit of pleasure, enjoyment, and sensory and emotional gratification.\\
4. Stimulation: Seeks novelty and challenge in life, valuing excitement, variety, and adventure.\\
5. Self-direction: Independent thought and action — choosing, creating, and exploring.\\
6. Universalism: Understanding, appreciation, tolerance, and protection for the welfare of all people and nature.\\
7. Benevolence: Preserving and enhancing the welfare of those with whom one is in frequent personal contact (the ‘in-group’).\\
8. Tradition: Respect, commitment, and acceptance of the customs and ideas that traditional culture or religion provide the self.\\
9. Conformity: Restraint of actions, inclinations, and impulses likely to upset or harm others and violate social expectations or norms.\\
10. Security: Safety, harmony, and stability of society, relationships, and the self. \\

Judgement: <judgement\_i>
\end{mdframed}

\caption{\brihi{add caption}}
\label{fig:prompt_shwartz}
\end{figure}

